Multipath TCP: Analysis, Design and Implementation

Multi-path TCP (MP-TCP) has the potential to greatly improve application performance by using multiple paths transparently. We propose a fluid model for a large class of MP-TCP algorithms and identify design criteria that guarantee the existence, uniqueness, and stability of system equilibrium. We clarify how algorithm parameters impact TCP-friendliness, responsiveness, and window oscillation and demonstrate an inevitable tradeoff among these properties. We discuss the implications of these properties on the behavior of existing algorithms and motivate a new design that generalizes existing algorithms and strikes a good balance among TCP-friendliness, responsiveness, and window oscillation. We have implemented our algorithm in the Linux kernel. We use our prototype to compare the new algorithm with existing MP-TCP algorithms.

==> figure/design_chart.tex <==
% Generated with LaTeXDraw 2.0.8
% Tue Oct 09 19:04:03 PDT 2012
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{0.8} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-1.99)(7.38,1.99)
\usefont{T1}{ptm}{m}{n}
\rput(1.39,1.42){\large Flow Level}
\usefont{T1}{ptm}{m}{n}
\rput(1.31,0.96){\large Stability}
\usefont{T1}{ptm}{m}{n}
\rput(5.81,1.36){\large Packet Level}
\usefont{T1}{ptm}{m}{n}
\rput(5.81,0.96){\large Stability}
\usefont{T1}{ptm}{m}{n}
\rput(1.46,-1.305){\Large Fairness}
\usefont{T1}{ptm}{m}{n}
\rput(5.91,-1.345){\Large Flap}
\psellipse[linewidth=0.04,dimen=outer](1.4,1.28)(1.4,0.71)
\psellipse[linewidth=0.04,dimen=outer](5.84,1.28)(1.4,0.71)
\psellipse[linewidth=0.04,dimen=outer](1.42,-1.28)(1.4,0.71)
\psellipse[linewidth=0.04,dimen=outer](5.92,-1.28)(1.4,0.71)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{<->}(2.78,1.31)(4.48,1.29)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{<->}(2.86,-1.27)(4.56,-1.29)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{<->}(1.4,0.53)(1.42,-0.65)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{<->}(5.86,0.57)(5.88,-0.61)
\usefont{T1}{ptm}{m}{n}
\rput(3.65,1.535){$k_r(x_s)$}
\usefont{T1}{ptm}{m}{n}
\rput(0.76,-0.0050){$f_r(x_s)$}
\usefont{T1}{ptm}{m}{n}
\rput(6.55,-0.085){$k_r(x_s)$}
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{<->}(2.46,0.79)(4.8,-0.75)
\usefont{T1}{ptm}{m}{n}
\rput(3.97,0.335){$k_r(x_s)$}
\usefont{T1}{ptm}{m}{n}
\rput(3.48,-0.285){$f_r(x_s)$}
\usefont{T1}{ptm}{m}{n}
\rput(3.72,-1.505){$f_r(x_s)$}
\end{pspicture} 
}



==> figure/top1.tex <==
% Generated with LaTeXDraw 2.0.8
% Wed Oct 10 14:09:00 PDT 2012
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{1} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-2.0)(12.74,2.04)
\definecolor{color506b}{rgb}{0.0,0.6,1.0}
\definecolor{color515}{rgb}{1.0,0.2,0.2}
\definecolor{color516}{rgb}{1.0,0.0,0.2}
\psline[linewidth=0.08cm](4.96,1.16)(7.82,1.14)
\psline[linewidth=0.08cm](5.04,-1.4)(7.82,-1.42)
\psellipse[linewidth=0.06,dimen=outer,fillstyle=solid,fillcolor=color506b](8.25,1.09)(0.35,0.37)
\usefont{T1}{ptm}{m}{n}
\rput(6.42,1.445){\Large $c_1, \tau_1$}
\psline[linewidth=0.06cm,linecolor=red,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.96,1.1)(4.28,1.1)
\psline[linewidth=0.06cm,linecolor=color515,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.98,1.08)(4.26,-1.38)
\psline[linewidth=0.06cm,linecolor=color516,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.64,1.14)(10.78,1.14)
\psline[linewidth=0.06cm,linecolor=red,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.66,-1.44)(10.8,1.02)
\psline[linewidth=0.06cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.92,-1.44)(4.22,-1.46)
\psline[linewidth=0.06cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.76,-1.46)(10.84,-1.46)
\usefont{T1}{ptm}{m}{n}
\rput(1.0,1.185){\Large MP-TCP}
\usefont{T1}{ptm}{m}{n}
\rput(3.58,1.345){\Large $x_1$}
\usefont{T1}{ptm}{m}{n}
\rput(3.58,0.125){\Large $x_2$}
\usefont{T1}{ptm}{m}{n}
\rput(3.42,-1.215){\Large $x_3$}
\psellipse[linewidth=0.06,dimen=outer,fillstyle=solid,fillcolor=color506b](8.25,-1.43)(0.35,0.37)
\psellipse[linewidth=0.06,dimen=outer,fillstyle=solid,fillcolor=color506b](4.61,1.11)(0.35,0.37)
\psellipse[linewidth=0.06,dimen=outer,fillstyle=solid,fillcolor=color506b](4.67,-1.51)(0.35,0.37)
\usefont{T1}{ptm}{m}{n}
\rput(1.04,0.725){\Large Flows}
\psframe[linewidth=0.04,dimen=outer](1.96,1.62)(0.06,0.5)
\pscustom[linewidth=0.04]
{
\newpath
\moveto(2.46,1.54)
\lineto(2.54,1.21)
\curveto(2.58,1.045)(2.58,0.715)(2.54,0.55)
\curveto(2.5,0.385)(2.435,0.205)(2.41,0.19)
\curveto(2.385,0.175)(2.345,0.155)(2.3,0.14)
}
\usefont{T1}{ptm}{m}{n}
\rput(0.89,-1.315){\Large SP-TCP}
\usefont{T1}{ptm}{m}{n}
\rput(0.98,-1.775){\Large Flows}
\psframe[linewidth=0.04,dimen=outer](1.9,-0.88)(0.0,-2.0)
\usefont{T1}{ptm}{m}{n}
\rput(11.78,1.185){\Large MP-TCP}
\usefont{T1}{ptm}{m}{n}
\rput(11.82,0.725){\Large Flows}
\psframe[linewidth=0.04,dimen=outer](12.74,1.62)(10.84,0.5)
\usefont{T1}{ptm}{m}{n}
\rput(11.67,-1.315){\Large SP-TCP}
\usefont{T1}{ptm}{m}{n}
\rput(11.76,-1.775){\Large Flows}
\psframe[linewidth=0.04,dimen=outer](12.68,-0.88)(10.78,-2.0)
\pscustom[linewidth=0.04]
{
\newpath
\moveto(10.54538,0.10933014)
\lineto(10.350933,0.3877002)
\curveto(10.253709,0.5268854)(10.133792,0.8343265)(10.111098,1.0025824)
\curveto(10.088406,1.170838)(10.083552,1.3621533)(10.101393,1.3852124)
\curveto(10.119233,1.4082714)(10.149231,1.4414399)(10.185704,1.4717667)
}
\usefont{T1}{ptm}{m}{n}
\rput(6.44,-1.035){\Large $c_2, \tau_2$}
\usefont{T1}{ptm}{m}{n}
\rput(1.06,1.81){\large $N_1$}
\usefont{T1}{ptm}{m}{n}
\rput(1.02,-0.67){\large $N_2$}
\end{pspicture} 
}



==> figure/top1_capacity.tex <==
% Generated with LaTeXDraw 2.0.8
% Wed Oct 10 14:11:13 PDT 2012
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{0.5} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-2.82)(10.38,2.82)
\definecolor{color556}{rgb}{0.2,0.4,1.0}
\psline[linewidth=0.08cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.32,-2.32)(0.34,2.48)
\psline[linewidth=0.08cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.28,-2.28)(9.88,-2.28)
\psline[linewidth=0.12cm,linecolor=color556](4.54,1.86)(8.72,-2.3)
\psdots[dotsize=0.4](4.5,1.84)
\psline[linewidth=0.08cm,linestyle=dashed,dash=0.16cm 0.16cm](0.34,1.84)(4.46,1.82)
\psline[linewidth=0.08cm,linestyle=dashed,dash=0.16cm 0.16cm](4.5,1.84)(4.52,-2.3)
\usefont{T1}{ptm}{m}{n}
\rput(4.47,-2.605){\LARGE 1}
\usefont{T1}{ptm}{m}{n}
\rput(0.03,1.775){\LARGE 1}
\usefont{T1}{ptm}{m}{n}
\rput(8.68,-2.565){\LARGE 2}
\usefont{T1}{ptm}{m}{n}
\rput(9.56,-1.905){\LARGE $c'_1$}
\usefont{T1}{ptm}{m}{n}
\rput(0.86,2.515){\LARGE $c'_2$}
\usefont{T1}{ptm}{m}{n}
\rput(5.64,2.275){\LARGE $(c_1,c_2)$}
\end{pspicture} 
}



==> figure/top2.tex <==
% Generated with LaTeXDraw 2.0.8
% Sat Oct 13 17:19:00 PDT 2012
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{0.35} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-5.4075146)(19.829784,5.4075146)
\definecolor{color2029b}{rgb}{0.2,0.6,1.0}
\definecolor{color2053}{rgb}{0.0,0.0,0.8}
\psline[linewidth=0.08cm,linecolor=red,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.103951,0.33248544)(7.023952,-1.6275146)
\psline[linewidth=0.08cm,linecolor=red,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.323952,0.89248544)(9.323952,2.8324854)
\rput{-180.0}(13.327904,0.0049708555){\pstriangle[linewidth=0.02,linecolor=blue,linestyle=dotted,dotsep=0.16cm,dimen=outer](6.663952,-5.0275145)(12.68,10.06)}
\rput{-90.0}(5.151801,8.207841){\pscircle[linewidth=0.08,dimen=outer](6.6798205,1.5280198){3.4065938}}
\rput{-90.0}(7.511976,8.831976){\psframe[linewidth=0.04,dimen=outer,fillstyle=solid](8.659491,1.171976)(7.6844616,0.14802407)}
\psline[linewidth=0.08cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(6.483952,3.2724855)(4.163952,3.2324855)
\psline[linewidth=0.08cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(7.063952,3.2724855)(9.203952,3.2324855)
\psline[linewidth=0.08cm,linecolor=blue,linestyle=dotted,dotsep=0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.063952,0.9324854)(3.9639518,2.7324855)
\psline[linewidth=0.08cm,linecolor=blue,linestyle=dotted,dotsep=0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.3639517,0.43248543)(6.763952,-1.5275146)
\rput{-90.0}(3.9320388,3.5775821){\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color2029b](3.7548106,-0.17722832){0.39028627}}
\psline[linewidth=0.08cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(6.3439517,5.0524855)(1.0839518,5.0124855)
\psline[linewidth=0.08cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.403952,0.11248543)(0.7039519,4.4324856)
\psline[linewidth=0.2cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.988558,4.4293857)(5.2448144,4.594105)
\psline[linewidth=0.2cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.339636,1.3387854)(3.324253,1.750809)
\psline[linewidth=0.2cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.381222,4.4578085)(8.686682,4.3071623)
\psline[linewidth=0.2cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(10.0639515,1.4924854)(10.043952,1.1124854)
\psline[linewidth=0.2cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.23202,-1.4504708)(7.981911,-1.6112351)
\psline[linewidth=0.2cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.1679235,-1.4983181)(4.890315,-1.3235795)
\usefont{T1}{ptm}{m}{n}
\rput(5.103952,4.1074853){\LARGE c}
\psline[linewidth=0.08cm,linecolor=red,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(7.143952,5.0524855)(12.303952,5.0124855)
\psline[linewidth=0.08cm,linecolor=red,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(9.783952,-0.047514573)(12.5639515,4.3724856)
\psline[linewidth=0.08cm,linecolor=blue,linestyle=dotted,dotsep=0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(9.323952,-0.7675146)(7.043952,-4.4275146)
\psline[linewidth=0.08cm,linecolor=blue,linestyle=dotted,dotsep=0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.863952,-0.6275146)(6.3239517,-4.4075146)
\psline[linewidth=0.2cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.3041086,5.0074635)(2.8237953,4.9975076)
\psline[linewidth=0.2cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.9952308,2.361324)(1.732673,2.7636466)
\psline[linewidth=0.2cm,linecolor=red,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(9.863986,5.0116982)(10.343918,5.0332727)
\psline[linewidth=0.2cm,linecolor=red,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(11.573657,2.7951047)(11.874247,3.169866)
\psline[linewidth=0.2cm,linecolor=color2053,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.366277,-2.370786)(8.121627,-2.784243)
\psline[linewidth=0.2cm,linecolor=color2053,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.1233025,-2.5627897)(5.404601,-2.9522395)
\usefont{T1}{ptm}{m}{n}
\rput(8.163952,0.62748545){\LARGE S2}
\usefont{T1}{ptm}{m}{n}
\rput(3.7839518,-0.21751457){\large R6}
\usefont{T1}{ptm}{m}{n}
\rput(2.2239518,-1.7125145){\LARGE Router}
\usefont{T1}{ptm}{m}{n}
\rput(2.7239518,-2.7325146){\LARGE Src or Dest}
\psline[linewidth=0.06cm](0.50395185,-3.4475145)(1.3839519,-3.4475145)
\psline[linewidth=0.12cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.0440269,-3.4636414)(1.2438768,-3.4713876)
\usefont{T1}{ptm}{m}{n}
\rput(2.133952,-3.4525146){\LARGE Link}
\rput{-90.0}(-4.408024,5.431976){\psframe[linewidth=0.04,dimen=outer,fillstyle=solid](0.9994905,5.431976)(0.024461364,4.408024)}
\usefont{T1}{ptm}{m}{n}
\rput(0.5239519,4.8874855){\LARGE D1}
\rput{-90.0}(7.951976,17.671976){\psframe[linewidth=0.04,dimen=outer,fillstyle=solid](13.299491,5.371976)(12.324461,4.348024)}
\usefont{T1}{ptm}{m}{n}
\rput(12.843952,4.8274856){\LARGE D2}
\rput{-90.0}(11.631976,1.791976){\psframe[linewidth=0.04,dimen=outer,fillstyle=solid](7.1994905,-4.408024)(6.2244616,-5.431976)}
\usefont{T1}{ptm}{m}{n}
\rput(6.673952,-4.9525146){\LARGE D3}
\rput{-90.0}(0.5920388,6.877582){\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color2029b](3.7348106,3.1427717){0.39028627}}
\usefont{T1}{ptm}{m}{n}
\rput(3.7839518,3.1224854){\large R1}
\rput{-90.0}(8.752039,4.957582){\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color2029b](6.8548107,-1.8972284){0.39028627}}
\usefont{T1}{ptm}{m}{n}
\rput(6.873952,-1.9375145){\large R5}
\rput{-90.0}(9.892038,9.177582){\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color2029b](9.53481,-0.3572283){0.39028627}}
\usefont{T1}{ptm}{m}{n}
\rput(9.583952,-0.39751458){\large R4}
\rput{-90.0}(6.4720387,12.717582){\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color2029b](9.5948105,3.1227717){0.39028627}}
\usefont{T1}{ptm}{m}{n}
\rput(9.613952,3.0824854){\large R3}
\rput{-90.0}(1.7520388,11.717582){\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color2029b](6.7348104,4.982772){0.39028627}}
\usefont{T1}{ptm}{m}{n}
\rput(6.763952,4.9424853){\large R2}
\rput{-90.0}(3.511976,10.031976){\psframe[linewidth=0.04,dimen=outer,fillstyle=solid](7.2594905,3.771976)(6.2844615,2.748024)}
\usefont{T1}{ptm}{m}{n}
\rput(6.743952,3.2274854){\LARGE S1}
\rput{-90.0}(4.451976,5.931976){\psframe[linewidth=0.04,dimen=outer,fillstyle=solid](5.6794906,1.2519759)(4.7044616,0.22802407)}
\usefont{T1}{ptm}{m}{n}
\rput(5.173952,0.70748544){\LARGE S3}
\rput{-90.0}(3.631976,-1.848024){\psframe[linewidth=0.04,dimen=outer,fillstyle=solid](1.1994905,-2.448024)(0.5844614,-3.031976)}
\rput{-90.0}(2.572039,-0.90241784){\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color2029b](0.8348105,-1.7372283){0.39028627}}
\usefont{T1}{ptm}{m}{n}
\rput(12.143951,1.1874855){\LARGE \psframebox[linewidth=0.04]{S1}}
\usefont{T1}{ptm}{m}{n}
\rput(19.243952,1.0674855){\LARGE \psframebox[linewidth=0.04]{D1}}
\usefont{T1}{ptm}{m}{n}
\rput(13.663952,1.7974855){\Large \pscirclebox[linewidth=0.04]{R1}}
\usefont{T1}{ptm}{m}{n}
\rput(17.683952,1.7774854){\Large \pscirclebox[linewidth=0.04]{R2}}
\usefont{T1}{ptm}{m}{n}
\rput(17.703953,0.37748542){\Large \pscirclebox[linewidth=0.04]{R6}}
\usefont{T1}{ptm}{m}{n}
\rput(13.693952,0.41748542){\Large \pscirclebox[linewidth=0.04]{R3}}
\usefont{T1}{ptm}{m}{n}
\rput(16.353952,0.41748542){\Large \pscirclebox[linewidth=0.04]{R5}}
\usefont{T1}{ptm}{m}{n}
\rput(15.023952,0.39748544){\Large \pscirclebox[linewidth=0.04]{R4}}
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(12.5639515,1.2324854)(13.283952,1.6924855)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(14.043952,1.8324854)(17.283953,1.8124855)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(12.583952,1.1124854)(13.303952,0.5924854)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(14.103951,0.47248542)(14.643951,0.47248542)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(15.443952,0.47248542)(15.983952,0.47248542)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(16.763952,0.45248544)(17.303951,0.45248544)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(18.123951,1.7124854)(18.763952,1.1924855)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(18.103952,0.41248542)(18.743952,0.9924854)
\usefont{T1}{ptm}{m}{n}
\rput(12.183952,-1.1925145){\LARGE \psframebox[linewidth=0.04]{S2}}
\usefont{T1}{ptm}{m}{n}
\rput(19.283953,-1.3125145){\LARGE \psframebox[linewidth=0.04]{D2}}
\usefont{T1}{ptm}{m}{n}
\rput(13.693952,-0.5825146){\Large \pscirclebox[linewidth=0.04]{R3}}
\usefont{T1}{ptm}{m}{n}
\rput(17.703953,-0.60251456){\Large \pscirclebox[linewidth=0.04]{R4}}
\usefont{T1}{ptm}{m}{n}
\rput(17.723951,-2.0025146){\Large \pscirclebox[linewidth=0.04]{R2}}
\usefont{T1}{ptm}{m}{n}
\rput(13.713952,-1.9625145){\Large \pscirclebox[linewidth=0.04]{R5}}
\usefont{T1}{ptm}{m}{n}
\rput(16.363953,-1.9625145){\Large \pscirclebox[linewidth=0.04]{R1}}
\usefont{T1}{ptm}{m}{n}
\rput(15.043952,-1.9825146){\Large \pscirclebox[linewidth=0.04]{R6}}
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(12.583952,-1.1475146)(13.303952,-0.68751454)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(14.0639515,-0.54751456)(17.303951,-0.5675146)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(12.603951,-1.2675146)(13.323952,-1.7875146)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(14.123952,-1.9075146)(14.663952,-1.9075146)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(15.463952,-1.9075146)(16.003952,-1.9075146)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(16.783953,-1.9275146)(17.323952,-1.9275146)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(18.143951,-0.66751456)(18.783953,-1.1875145)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(18.123951,-1.9675145)(18.763952,-1.3875146)
\usefont{T1}{ptm}{m}{n}
\rput(12.173952,-3.5525146){\LARGE \psframebox[linewidth=0.04]{S3}}
\usefont{T1}{ptm}{m}{n}
\rput(19.273952,-3.6725147){\LARGE \psframebox[linewidth=0.04]{D3}}
\usefont{T1}{ptm}{m}{n}
\rput(13.693952,-2.9425147){\Large \pscirclebox[linewidth=0.04]{R5}}
\usefont{T1}{ptm}{m}{n}
\rput(17.703953,-2.9625146){\Large \pscirclebox[linewidth=0.04]{R6}}
\usefont{T1}{ptm}{m}{n}
\rput(17.723951,-4.3625145){\Large \pscirclebox[linewidth=0.04]{R4}}
\usefont{T1}{ptm}{m}{n}
\rput(13.703952,-4.3225145){\Large \pscirclebox[linewidth=0.04]{R1}}
\usefont{T1}{ptm}{m}{n}
\rput(16.373951,-4.3225145){\Large \pscirclebox[linewidth=0.04]{R3}}
\usefont{T1}{ptm}{m}{n}
\rput(15.043952,-4.3425145){\Large \pscirclebox[linewidth=0.04]{R2}}
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(12.583952,-3.5075145)(13.303952,-3.0475147)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(14.0639515,-2.9075146)(17.303951,-2.9275146)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(12.603951,-3.6275146)(13.323952,-4.1475143)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(14.123952,-4.2675147)(14.663952,-4.2675147)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(15.463952,-4.2675147)(16.003952,-4.2675147)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(16.783953,-4.2875147)(17.323952,-4.2875147)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(18.143951,-3.0275145)(18.783953,-3.5475147)
\psline[linewidth=0.06cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(18.123951,-4.3275146)(18.763952,-3.7475145)
\usefont{T1}{ptm}{m}{n}
\rput(5.063952,-1.0125146){\LARGE c}
\usefont{T1}{ptm}{m}{n}
\rput(9.723952,1.3674854){\LARGE c}
\end{pspicture} 
}



==> texcode/5_simulation.tex <==
\section{Simulation}\label{sec:simulation}

\begin{figure}
  \centering
%  \includegraphics[width=\linewidth]{figure/top1.ps}\\
\input{figure/top1.tex}
  \caption{Network for simulations on TCP friendliness and responsiveness,
  with $N_1$ MP-TCP flows and $N_2$ single-path TCP flows sharing $2$ links of capacity $c_1$, $c_2$ and delay $\tau_1$, $\tau_2$. MP-TCP flows maintain two routes with rate $x_{1}$, $x_{2}$. Single-path TCP flows maintain one route with rate $x_{3}$.}\label{fig:top1}
\end{figure}

In this section we summarize our ns2 simulation results that illustrate the above analysis. 
Only the congestion avoidance phase on each path is modified to follow the MP-TCP
algorithm.  Every path follows the same slow start and loss recovery mechanism as
TCP-NewReno, except that the minimum {\it ssthresh} is set to $1$ instead of $2$ 
when more than $1$ path is available. 
We assume the advertised window \textit{awnd} is set to infinity. 

Our simulations are divided into three parts. 
First we compare TCP friendliness of our algorithm and prior algorithms. 
The result confirms that the Couple algorithm is the friendliest, ours is close to the Coupled
algorithm and friendlier than the other algorithms.
Second we compare the responsiveness of each algorithm in a dynamic environment
where flows come and go.  
The result shows that the Coupled algorithm is unresponsive (illustrating the tradeoff 
between responsiveness and friendliness).   EWTCP is the most responsive; ours is
similar in responsiveness but friendlier to single-path TCP flows.
Finally we show that all MP-TCP algorithms have smaller window oscillations than SP-TCP.

These simulations confirm our analytical results and suggest our design choice strike a 
good balance among friendliness, responsiveness, and window oscillation.

\subsection{TCP friendliness}



We study TCP friendliness of each algorithm using the network topology in Fig. \ref{fig:top1},
first with equal RTTs and then with different RTTs.
We assume all the flows are long lived and focus on the steady state throughput. 

\begin{table}
  \centering
    \caption{TCP friendliness (same RTTs): throughputs of MPTCP and single-path TCP users.}
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
               & ewtcp     & semi. & max    & ours &coupled \\\hline
%    Jain Fair Index & $0.80$    & $0.90$     & $0.92$           & $0.95$      &$1$         \\\hline
    MP-TCP Mbps & $2.98$ & $2.64$ & $2.58$ & $2.25$     &$2.22$     \\\hline
    SP-TCP Mbps  & $1.01$ & $1.32$ & $1.35$ & $1.61$   &$1.67$    \\\hline
  \end{tabular}
\label{table:top1}
\end{table}
In the first set of simulations, we let $\tau_1=\tau_2=20$ms, $c_1=c_2=10$Mbps 
and $N_1=N_2=5$. The average aggregate throughput of MP-TCP and 
single-path TCP users are shown in Table \ref{table:top1}. 
The EWTCP, Semicoupled and Max algorithms are significantly less friendly to SP-TCP.
The Coupled algorithm is the friendliest and our algorithm is very close.




%The above example shows the interaction between MP-TCP and single-path TCP users and it confirms our analysis of the fairness property in section \ref{subsec:fairness}. In the next example, we will show the interactions between different MP-TCP flows. Fig. \ref{fig:top2} shows a network topology with bottleneck link capacity $c=10$Mbps and $20$ms delay; the capacity of the rest of the links are large enough that it does not affect throughput. There are $3$ sets of source-destination pairs and there are $5$ MPTCP flows for each set of source destination pairs. The average throughput of MPTCP flows are shown in Table \ref{table:top2}. 
%
%
%According to Table \ref{table:top2}, our algorithm is still close to Coupled algorithm and the throughput of other algorithms are low. In the ideal case, each MP-TCP flow gets $2$Mbps throughput and there is no traffic on the second subpath for all the MP-TCP flows. Again, the minimal window size is $1$ for each subpath and this ideal state can not be achieved. In this example, deploying MP-TCP can decrease the throughput compared to the scenario where all the users switch back to single-path TCP. It means that two MPTCP flows may negatively affect each other and decrease the throughput of both of them. But we do not know how to minimize this negative effect, therefore interaction among multipath flows needs to be studied in the future. 

In the second set of simulations the link capacities and the number of flows are unchanged
but the propagation delays are changed to $\tau_1=10$ms and $\tau_2=50$ms. Due to space limitation we only show the throughput trajectories of the Max algorithm and ours, in Fig. \ref{fig:heterogeneous_rtt}. Compared with the simulation results obtained where each path has similar round trip time, Max algorithm become more unfriendly towards single-path TCP. However, our algorithm is quite moderate in 
comparison with the Max algorithm.

%The friendliness behavior of the algorithms is similar to the case with equal RTTs.
%Due to space limitation we only show the throughput trajectories of the Max algorithm
%and ours, in Fig. \ref{fig:heterogeneous_rtt}.   Our algorithm is quite moderate in 
%comparison with the Max algorithm.




%\begin{figure}
%  \centering
%%  \includegraphics[width=0.6\linewidth]{figure/top2.eps}\\
%\input{figure/top2.tex}
%  \caption{Network with $3$ set of source destination pairs with MP-TCP and each source enable $2$ subpaths. The bottleneck links are specified with capacity $c$. The two subpaths for each source is explicitly expressed in the right side.}\label{fig:top2}
%\end{figure}
%\begin{table}
%  \centering
%  \caption{Throughput of MP-TCP users. }
%  \begin{tabular}{|c|c|c|c|c|c|}
%    \hline
%         &       ewtcp     & semi. & max     & ours &coupled \\\hline
%Througput Mbps    &  $1.32$ & $1.43$ & $1.45$ & $1.72$     &$1.78$     \\\hline
%  \end{tabular}
%\label{table:top2}
%\end{table}

\subsection{Responsiveness}\label{sim:responsive}

\begin{figure}
\centering
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=\linewidth,height=0.7\linewidth]{figure/top1_s_damon_heter_each.pdf}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=\linewidth,height=0.7\linewidth]{figure/top1_s_damon_heter_total.pdf}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=\linewidth,height=0.7\linewidth]{figure/top1_s_ours_heter_each.pdf}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=\linewidth,height=0.7\linewidth]{figure/top1_s_ours_heter_total.pdf}
\end{minipage}
\caption{TCP friendliness (different RTTs): the throughputs of MP-TCP and single-path TCP 
users.  Left panel: throughput of each path.  Right panel: aggregate throughput of each source. }
\label{fig:heterogeneous_rtt}
\end{figure}

A good algorithm should react fast in a dynamic environment.
We use the network in Fig. \ref{fig:top1} with $c_1=c_2=2$Mbps, $\tau_1=\tau_2=20$ms 
and $N_1=N_2=1$. The MP-TCP flow is long lived while the SP-TCP flow 
starts at $40$s and end at $80$s. We record the average throughput of the SP-TCP
flow from 40-80s, which measures the friendliness of MP-TCP. 
We also measure the time for the throughput on the second path to recover\footnote{Defined as 
the first time the throughput on the second path is within $90\%$ of the average throughput 
after the single-path user has left.} for MP-TCP users. 
It measures the responsiveness of MP-TCP.
These measurements are shown in Table \ref{table:top1_d} and the throughput trajectories of all algorithms are shown in Fig. \ref{fig:dynamic}.
\begin{table}
  \centering
  \caption{Responsiveness: convergence time of MP-TCP and throughput of single-path TCP}
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         &       ewtcp     & semi. & max     & ours &coupled \\\hline
 Convergence time (s)    &  $1.0$ & $2.5$ & $4.5$ & $4.5$     &$54.0$     \\\hline
SP-TCP througput (Mbps)   &  $1.02$ & $1.17$ & $1.30$ & $1.57$     &$1.72$     \\\hline
  \end{tabular}
%  \caption{Time to converge when the single-path TCP user leave after $80$s and the average throughput for single-path TCP users during $40$s to $80$s. The network topology is shown in Fig.(\ref{fig:top1}) with $\tau_1=\tau_2=20$ms and $c_1=c_2=2$Mbps.}
\label{table:top1_d}
\end{table}
EWTCP is the most responsive among all the algorithms.   Ours is as responsive as 
the Max algorithm, yet significantly friendlier than EWTCP.
The Coupled algorithm took an excessively long time to recover. The excessively slow recovery of the throughput on the second path (see Fig. \ref{fig:dynamic}) is due to the design of Coupled algorithm that increases the window by $w_r/(\sum_{k\in s} w_k)^2$ on each ACK.  After the single-path TCP flow has left, $w_2$ is small while $w_1$ is large, so that $w_2/(w_1+w_2)^2$ is very small.  It therefore takes a long time for $w_2$ to increase to its steady state value.  In general, under the Coupled algorithm, a route with a large throughput can greatly suppress the throughput on another route even though the other route is underutilized.

\begin{figure}
\centering
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=\linewidth,height=0.7\linewidth]{figure/packet_stability.pdf}
\label{fig:packet_stability_mptcp}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=\linewidth,height=0.7\linewidth]{figure/packet_stability_reno.pdf}
\label{fig:packet_stability_reno}
\end{minipage}
\caption{Window oscillation: the red trajectories represent throughput fluctuations
	experience by the application that run on MP-TCP/SP-TCP.}
\label{fig:packet_stability}
\end{figure}

  
\begin{figure*}[!htbp]
\centering
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_ewtcp_single.pdf}
\label{fig:top1_d_ewtcp_single}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_semi_single.pdf}
\label{fig:top1_d_semi_single}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_damon_single.pdf}
\label{fig:top1_d_damon_single}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_ours_single.pdf}
\label{fig:top1_d_ours_single}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_couple_single.pdf}
\label{fig:top1_d_coupled_single}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_ewtcp_sum.pdf}
\label{fig:top1_d_ewtcp_sum}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_semi_sum.pdf}
\label{fig:top1_d_semi_sum}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_damon_sum.pdf}
\label{fig:top1_d_damon_sum}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_ours_sum.pdf}
\label{fig:top1_d_ours_sum}
\end{minipage}
\begin{minipage}[b]{0.195\linewidth}
\includegraphics[width=1\linewidth,height=0.8\linewidth]{figure/top1_d_couple_sum.pdf}
\label{fig:top1_d_coupled_sum}
\end{minipage}
\caption{Responsiveness: dynamic behavior of MP-TCP. 
Upper figures:  throughput trajectory for each path.  
Lower figures:  total throughput for each user.
}
\label{fig:dynamic}
\end{figure*}
%\slow{Qiuyu: can you rep lot the lower figures in Fig \ref{fig:dynamic}
%so that SP-TCP trajectories are also in 	red, as in upper figures?}



\subsection{Window oscillation}


We use a single-link network model to compare window oscillation under MP-TCP
and that under SP-TCP.  
First a MP-TCP flow initiates two subpaths through that link, and
we measure the window size of each subpath and their aggregate window size.
Then a TCP-NewReno flow traverse the same link and we measure its window size. 
 The results are shown in Fig. \ref{fig:packet_stability} for our algorithm in comparison
 with SP-TCP (other MP-TCP algorithms have a similar behavior).  They confirm
 that enabling multiple paths reduces window oscillation.



%\begin{figure}[htbp]
%\centering
%\begin{minipage}[b]{0.49\linewidth}
%\includegraphics[width=\linewidth,height=0.7\linewidth]{figure/flap_coupled}
%\end{minipage}
%\begin{minipage}[b]{0.49\linewidth}
%\includegraphics[width=\linewidth,height=0.7\linewidth]{figure/flap_our}
%\end{minipage}
%  \caption{The probability distribution of window sizes subpath 1 when $2$ paths share a bottleneck link using Monte Carlo simulation. $x$ axis is normalized to be $1$ and one path is plot due symmetry.}\label{fig:flappiness_ours}
%\end{figure}

%Next, we test whether our algorithm is flappy. We have already predicted that our algorithm is not flappy by our sufficient condition in Theorem \ref{thm:6}. Here we will verify our prediction by simulations. Consider the same toy model in section 5. To verify our prediction, two subpaths of a user share a bottleneck link with bandwidth $100$pkts. Therefore either $w_1$ or $w_2$'s packets will be dropped when $w_1+w_2\geq 100$. We compare our algorithm with Coupled algorithm and the result is shown in Fig. (\ref{fig:flappiness_ours}). Although there are some spikes in the probability mass function of window size, the probability still decrease instead of increasing when either $w_1$ or $w_2$ is small. 


%\begin{figure}[!htb]
%\centering
%  \includegraphics[width=\linewidth,height=0.3\linewidth]{figure/flap_ours.eps}\\
%  \caption{Flappiness of Max and our algorithm.}\label{fig:flappiness_ours}
%\end{figure}

==> texcode/6_conclusion.tex <==
\section{Conclusion}\label{sec:conc}

We have presented a model for MP-TCP and identified designs that guarantee the existence, uniqueness and stability of the network equilibrium. 
We have characterized the design space and study the tradeoff 
among TCP friendliness, responsiveness, and window oscillation. 
We have proposed a new MP-TCP algorithm that generalizes existing
algorithms and strikes a good balance among these properties.
We have presented preliminary ns2 simulations to illustrate our 
analysis.

%In this paper, we investigate the emerging problems in designing MP-TCP congestion control algorithms. We show the existence, uniqueness and stability properties of the equilibria under a unified model of MP-TCP algorithms using a new approach. Furthermore, we characterize the design space and study the tradeoffs among various performance metrics. Finally, we design a new MP-TCP algorithm and compare its performance
%with existing algorithms through ns2 simulation.

%The limitation of this work is that we did not incorporate the feedback delay into consideration when we analyze the convergence performance. In addition,  we only consider the impact of MP-TCP flows on SP-TCP flows when we study the fairness of MP-TCP algorithms. We need more understanding of the interactions among MP-TCP flows, e.g. two MP-TCP flows may interact in some ways such that both of their throughput decreases. 

